Inside the Visual Mind: Neuroscience-Motivated Concept Circuits for Interpreting and Steering Vision Transformers

Despite high accuracy, Vision Transformer (ViT) predictions can be driven by spurious cues, raising the need to understand their inner workings before safe deployment. Sparse autoencoders (SAEs) provide a promising lens for decomposing model representations into human-interpretable concepts, yet adapting SAE-based interpretation to ViTs remains challenging due to limited control over concept coverage and subjective, non-scalable feature interpretation. To fill the gaps, motivated by neuroscience-inspired principles, we propose ViSAE, a mechanistic interpretability toolbox for understanding ViT inner workings through concept circuits. ViSAE consists of three components: (1) A probing suite with 64K images and a 16K visually grounded concept vocabulary, improving concept coverage efficiency by 20x over ImageNet and interpretation accuracy by 28.7% over existing concept sets. (2) Top-down concept reading and Bottom-up circuit tracing algorithms that automatically recover ViT inner workings via concept circuits. (3) Applications for auditing and steering ViT behavior. Through concept editing, ViSAE improves the worst-group accuracy on WaterBirds by 48.2%, outperforming existing methods by 23.8%. Our data and code: https://github.com/deep-real/ViSAE.

==> fig/information_flow_full.tex <==
\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{1.8in} \rule{0.95\linewidth}{0pt}}
   % \includegraphics[width=0.98\linewidth]{img/information_flow.pdf}
   % \vspace{-15pt}
   \caption{
   Full information flow graph.
   }
   % \vspace{-15pt}
   \label{fig:information_flow_full}
\end{figure}

==> fig/localization_additional.tex <==
\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{1.0in} \rule{0.95\linewidth}{0pt}}
   % \includegraphics[width=1.0\linewidth]{img/localization.pdf}
   % \vspace{-15pt}
   \caption{
   Concept localization
   }
   % \vspace{-15pt}
   \label{fig:localization_additional}
\end{figure}

==> fig/spurious_correlation_additional.tex <==
% \begin{wrapfigure}{r}{0.6\textwidth}
% \vspace{-18pt}
\begin{figure}[ht]
    \centering
  % \begin{center}
  \fbox{\rule{0pt}{2.2in} \rule{0.95\linewidth}{0pt}}
  % \includegraphics[width=0.6\textwidth]{img/failure_mode.pdf}
  % \end{center}
  % \captionsetup{justification=raggedright, font=it}
  \vspace{-8pt}
  \caption{
  Qualitative examples of steering on WaterBird dataset.
  }
  \label{fig:spurious_correlation_additional}
\end{figure}

% \vspace{-15pt}
% \end{wrapfigure}

==> tab/eval_neuroscience.tex <==
% \begin{table}[t]
% \resizebox{1.0\columnwidth}{!}{%
% \begin{tabular}{cccccc}
% \hline
% SAE Training Data & \# of Images & Recon. Err. $\downarrow$ & Monosematicity $\uparrow$ & Decoder Orth. $\downarrow$ & Dead Neurons $\downarrow$ \\ \hline
% ImageNet          & 1,281K       & 0.032                    & 0.563                     & 0.032                      & 0.000                     \\
% ImageNet (DS+RR)  & 65K          & 0.039                    & 0.489                     & 0.041                      & 0.000                     \\
% Ours              & 64K          & \textbf{0.026}           & \textbf{0.590}            & \textbf{0.030}             & 0.000                     \\ \hline
% \end{tabular}
% }
% \end{table}

\begin{table}[t]
\centering
\caption{Evaluation on the Effectiveness of Neuroscience-Motivated Design}
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{cccc}
\toprule[1pt]
SAE Training Data          & ImageNet & ImageNet (DS+RR) & Ours           \\ \midrule[0.5pt]
\# of Images               & 1,281K   & 65K              & 64K            \\ \midrule[0.75pt]
Recon. Err. $\downarrow$   & 0.032    & 0.039            & \textbf{0.026} \\
Monosemanticity $\uparrow$  & 0.563    & 0.489            & \textbf{0.590} \\
Decoder Orth. $\downarrow$ & 0.032    & 0.041            & \textbf{0.030} \\
Dead Neurons $\downarrow$  & 0.000    & 0.000            & 0.000          \\ \bottomrule[1pt]
\end{tabular}
}
\label{tab:eval_neuroscience}
\end{table}

==> tab/human_eval.tex <==
\begin{table}[]
\begin{tabular}{ccc}
\hline
Evaluator & Faithfulness    & Completeness    \\ \hline
Human_A   & 4.65 $\pm$ 0.06 & 4.72 $\pm$ 0.04 \\
Human_B   & 4.83 $\pm$ 0.20 & 4.73 $\pm$ 0.06 \\
Human_C   & 4.90 $\pm$ 0.05 & 4.78 $\pm$ 0.18 \\
Avg.      & 4.79            & 4.74            \\ \hline
\end{tabular}
\end{table}
